Numerical analysis of a hybrid method for radiation transport

In this work, we prove rigorous error estimates for a hybrid method introduced in [15] for solving the time-dependent radiation transport equation (RTE). The method relies on a splitting of the kinetic distribution function for the radiation into uncollided and collided components. A high-resolution method (in angle) is used to approximate the uncollided components and a low-resolution method is used to approximate the the collided component. After each time step, the kinetic distribution is reinitialized to be entirely uncollided. For this analysis, we consider a mono-energetic problem on a periodic domains, with constant material cross-sections of arbitrary size. To focus the analysis, we assume the uncollided equation is solved exactly and the collided part is approximated in angle via a spherical harmonic expansion ($\text{P}_N$ method). Using a non-standard set of semi-norms, we obtain estimates of the form $C(\varepsilon,\sigma,\Delta t)N^{-s}$ where $s\geq 1$ denotes the regularity of the solution in angle, $\varepsilon$ and $\sigma$ are scattering parameters, $\Delta t$ is the time-step before reinitialization, and $C$ is a complicated function of $\varepsilon$, $\sigma$, and $\Delta t$. These estimates involve analysis of the multiscale RTE that includes, but necessarily goes beyond, usual spectral analysis. We also compute error estimates for the monolithic $\text{P}_N$ method with the same resolution as the collided part in the hybrid. Our results highlight the benefits of the hybrid approach over the monolithic discretization in both highly scattering and streaming regimes.

==> sections/consistency.tex <==
\section{Interpolation error analysis}
In this section, we estimate the interpolation errors which appeared in the error estimates for the transport and hybrid models in Sections \ref{sec:pn_error} and \ref{sec:hybrid_error}. The error results therein were in terms of the best approximation in $L^2(\mathbb{S}^2)$ to the solution of the continuous solutions $\psi$ and $\psic$, respectively, and their gradients. This does not allow for a direct comparison of the method errors, nor does it provide insight into how often one should remap with the hybrid model to obtain comparable accuracy to the transport model. We need to estimate these in terms of the problem data. To this end, we first recall an interpolation estimate which relates the error in the angle discretization to higher order Sobolev semi-norms of the solution. Then, assuming regular solutions exist, we use the evolution equations to estimate these semi-norms for the transport equation in Section \ref{sec:angle_reg_transport} and the hybrid model in Section \ref{sec:angle_reg_hybrid}.
\begin{lem}[Approximation properties, Corollary 2.7, pp 2652 in \cite{li2014spectral}]\label{lem:approx_prop}
For a function $f \in H^s(\mathbb{S}^2)$,
\begin{equation}
     \norma{\psi - P_N\psi} \leq c(s)N^{-s} |\psi|_{H^s(\mathbb{S}^2)}.
\end{equation}
\end{lem}
The semi-norm is given in terms of the three Euler angular derivatives:
\begin{equation}
    |\psi|_{H^s(\mathbb{S}^2)} := \sum_{1 \leq i < j \leq 3} \norma{D^s_{i,j}\psi}.
\end{equation}
The differential operators $D_{i,j}$ yield the rate of change along the intersection of the $x_i$-$x_j$ plane and the sphere. For example, in spherical coordinates we have $(\zeta_1, \zeta_2, \zeta_3) = (\sqrt{1-\zeta_3^2}\cos \theta, \sqrt{1-\zeta_3^2}\sin \theta,\zeta_3)$. Differentiation along the $x_1-x_2$ axis is simply
\begin{equation}
D_{1,2}^r f(\zeta) = \left(-\frac{\partial}{\partial \theta}\right)^r f(\zeta).
\end{equation}
To facilitate ease of analysis, we assume solutions are smooth enough that we can directly differentiate the evolution equations to obtain energy estimates for the higher order derivatives. A more technical analysis with fewer regularity assumptions to obtain similar estimates will be the subject of future research.
\begin{lem}[Basic angular derivative result\label{lem:partial_angle_omega}]
Let $\|\cdot\|_{\mathbb{R}^3}$ be the usual Euclidian norm in $\R^3$. Then for any $i, j$ and integer $r\geq 0$, 
\begin{equation}
\|\partial_{\theta}^r\Omega\|_{\R^3} \leq 1.
\end{equation}
\end{lem}
\begin{proof}
The conclusion follows from the definition of $\partial_{\theta}$ and the fact that the derivatives of $\cos\theta$ and $\sin\theta$ are always bounded by $1$.
\end{proof}
%________________________________________________________________________________________________________________________
%_____________________________________________________________________________________________________________________________
\subsection{Angular derivative estimates for the transport model\label{sec:angle_reg_transport}}
 Define
\begin{equation}
    \norma{D^2 \psi} = \sqrt{d} \sum_{i,j}\norma{\partial_{x_i}\partial_{x_j}\psi}^2,
\end{equation}
i.e., the Frobenius norm of the Hessian matrix scaled by the square root of the dimension.
\begin{defn} \label{def:kappa_gamma} Given $t \in\mathbb{R}$, we define 
\begin{equation}
    \kappa(t)\equiv e^{-\sigma t}\quad\text{and}\quad \gamma(t)\equiv\frac{1-e^{-\sigma t}}{\sigma t}.
\end{equation}
\end{defn}
\begin{lem}[Regularity for the non-splitting model]\label{lem:nonsplitting_reg}
Let $\psi$ be the solution to \eqref{eq:scaled_transp}, and assume that the solution is $C^1$ in time and $C^{3}(\mathbb{T}^3)\cap C^1(\sphe)$, then for any $i,j$, and $g$ and $q$ smooth enough,
\begin{equation}\label{eq:regularity_original}
\norma{\partial_{\theta}\psi(t)}\leq  \norma{\partial_{\theta}g}\kappa(t)+\left[\norma{\partial_x g}+\norma{\partial_{\theta}q}_{\infty}\right]\gamma(t)t+\norma{\partial_x q}_{\infty}\left[1-\gamma(t)\right]\frac{t}{\sigma} 
\end{equation}
now if we bump up $\psi$ to a function in $C^1([0,T];C^{3}(\mathbb{T}^3)\cap H^1(\sphe))$, then
\begin{equation}\label{eq:reg_grad_ns}
\norma{\nabla_x\partial_{\theta}\psi(t)}\leq  \norma{\nabla_x\partial_{\theta}g}\kappa(t)+\left[\norma{D^2_xg}+\norma{\nabla_x\partial_{\theta}q}_{\infty}\right]\gamma(t)t+\norma{D^2_xq}_{\infty}\left[1-\gamma(t)\right]\frac{t}{\sigma} 
\end{equation}
\end{lem}
\begin{proof}
Differentiation with respect to $\theta$ gives us 
	\begin{equation*}
		\begin{cases}
			\partial_t\left(\partial_{\theta}\psi\right)+\Omega\cdot\nabla_x\left(\partial_{\theta}\psi\right)+\sigma\partial_{\theta}\psi=\partial_{\theta}q-\partial_{\theta}\Omega\cdot\nabla_x\psi\\
			\left.\partial_{\theta}\psi\right|_{t=0}=\partial_{\theta}g.
		\end{cases}
	\end{equation*}
Applying Lemma \ref{lem:basic_stability_result} part \ref{lem:unc}, with $t_0=0,\,\zeta=\partial_{\theta}\psi$ and $Q=\partial_{\theta}q-\partial_{\theta}\Omega\cdot\nabla_x\psi$, Lemma \ref{lem:partial_angle_omega}, and  Lemma \ref{lem:nonsplitting_bound}, we can conclude that
	\begin{align*}
		\norma{\partial_{\theta}\psi(t)}&\leq e^{-\sigma t}\norma{\partial_{\theta}g}+\int_{0}^t e^{-\sigma( t-\omega)}\left[\norma{\partial_{\theta}q}_{\infty}+(\norma{\partial_x g}+\omega\norma{\partial_x q}_{\infty})\right]\,d\omega.
	\end{align*}
The conclusion follows by direct integration and Definition \ref{def:kappa_gamma}.

It is not hard to see that by Lemma \ref{lem:nonsplitting_bound}, that
\begin{equation*}
    \norma{D^2_x\psi(t)}\leq\norma{D^2_x g}+t\norma{D^2_xq}_{\infty}.
\end{equation*}
By applying  $\partial_\theta$ and $\nabla_x$ gives us 
	\begin{equation*}
	\partial_t\left(\nabla_x\partial_{\theta}\psi\right)+\nabla_x(\Omega\cdot\nabla_x\partial_{\theta}\psi+\partial_\theta\Omega\cdot\nabla_x\psi)+\sigma\nabla_x\partial_{\theta}\psi=\nabla_x\partial_{\theta}q,
	\end{equation*}
the conclusion follows by the same lines as above. 
\end{proof}
%______________________________________________________________________________________________________________________________________________________
\subsection{Angle derivative estimates for the hybrid model\label{sec:angle_reg_hybrid}}
Because the cross-sections do not depend on space, we can extend the results of Theorem \ref{thm:stability} to obtain a'priori estimates for higher order seminorms for smooth solutions. In particular, we can show for $\psium{}$,$\psicm{}\in C^3(X)$ the following:
\todo{Victor : clean up}
\begin{lem}\label{lem:hessian_est}
For all $m>0$ and $t\in [t_m,t_{m+1})$, we have (fill in more preconditions)
\begin{equation}
    \norma{D_x^2 \psicm{m}(t)} \leq  \kcm{m} (t)\norma{D_x^2 g} +  (\gcm{m} (t)(t-t_m) + \kcm{m} (t)t_m)\norma{D_x^2 q}_{\infty} .
\end{equation}
\end{lem}
Now assume we can classically differentiate the PDE by $x$ and $\theta$. This yields
\begin{equation}
    \partial_t \nabla_x \partial_{\theta} \psicm{m}(t) + \nabla_x\left( \Omega\cdot\nabla_x \partial_{\theta}\psicm{m} + \partial_{\theta}\Omega\cdot\nabla_x \psicm{m}  \right) 
    + \sigma\nabla_x \partial_{\theta} \psicm{m}(t) = 0.
\end{equation}
Taking the inner product with $\nabla_x\partial_{\theta}\psi_{c,m}$ and integrating by parts, we obtain
\begin{gather}
    \frac{1}{2}\frac{d}{dt}\norma{\nabla_x \partial_{\theta}\psicm{m}}^2 + \sigma \norma{\partial_x \partial_{\theta}\psicm{m}}^2 = - \left( \nabla_x \left(\partial_{\theta}\Omega\cdot \nabla_x \psicm{m}\right) , \nabla_x \partial_{\theta} \psicm{m} \right) 
    \\
    \leq \norma{D^2 \psi}\norma{\partial_x \partial_{\theta}\psicm{m}}.
\end{gather}
Thus,
\begin{gather}
    \frac{d}{dt}\norma{\nabla_x \partial_{\theta}\psicm{m}} + \sigma \norma{\partial_x \partial_{\theta}\psicm{m}} 
    \leq \norma{D_x^2 \psi}.
\end{gather}
Thus,
\begin{gather}
    \norma{\nabla_x \partial_{\theta}\psicm{m}(t)} 
    \leq e^{-\sigma t}\int_{t_m}^t e^{\sigma s}\norma{D_x^2 \psi(s)}.
\end{gather}
Up until the above equation, we only needed to assume $\psi \in C^2(X)\cap C^1(\mathbb{S}^2)$. For Lemma \ref{lem:hessian_est} to apply, we need to bump this up to $\psi \in C^3(X)\cap C^1(\mathbb{S}^2)$. Assume this and apply the lemma,
\begin{gather}
    \norma{\nabla_x \partial_{\theta}\psicm{m}(t)} 
    \leq e^{-\sigma t}\int_{t_m}^t e^{\sigma s}\left(\kcm{m} (s)\norma{D_x^2 g} +  (\gcm{m} (s)(s-t_m) + \kcm{m} (s)t_m)\norma{D_x^2 q}_{\infty}\right)ds.
\end{gather}
To integrate this exactly, we only need to focus on
\begin{align}
  \text{I,} & \quad\quad e^{-\sigma t}\int_{t_m}^t e^{\sigma s}  \kcm{m} (s) ds,\\
  \text{II,} & \quad\quad e^{-\sigma t}\int_{t_m}^t e^{\sigma s}  \gcm{m} (s)(s-t_m) ds.
\end{align}
For integral I, we note
\begin{equation}
    \left( \frac{1}{\sigma}e^{\sigma s} \kcm{m}(s) \right)' = e^{\sigma s}\kcm{m}(s) + e^{\sigma s}e^{-\sigma (s-t_m)} = e^{\sigma s}\kcm{m}(s) + e^{\sigma t_m}.
\end{equation}
Thus,
\begin{gather}
    e^{-\sigma t}\int_{t_m}^t e^{\sigma s}  \kcm{m} (s) ds =  \left( \frac{1}{\sigma}e^{-\sigma (t-s)} \kcm{m}(s) \right)\bigg|_{t_m}^{t} - \int_{t_m}^t e^{-\sigma(t-t_m)}ds
    \\
    =\frac{1}{\sigma} \kcm{m}(t) - (t-t_m)e^{-\sigma(t-t_m)} = \frac{(t-t_m)}{\sigma(t-t_m)}\left( \kcm{m}(t) - \sigma(t-t_m)e^{-\sigma(t-t_m)} \right)
    \\
    =(t-t_m)\frac{ 1-e^{-\tau} - \tau e^{-\tau}}{\tau}.
\end{gather}
where $\tau = \tau(t) = \sigma(t-t_m)$.

Now we integrate II.
\begin{gather}
    e^{-\sigma t}\int_{t_m}^t e^{\sigma s}  \gcm{m} (s)(s-t_m) ds = e^{-\sigma (t-t_m)}\int_{t_m}^t e^{\sigma (s-t_m)}  \gcm{m} (s)(s-t_m) ds
    \\
    =\frac{e^{-\sigma (t-t_m)}}{\sigma}\int_{t_m}^t e^{\sigma (s-t_m)}  \left(1-\frac{1-e^{-\sigma(s-t_m)}}{\sigma(s-t_m)}\right)\sigma(s-t_m) ds
    \\
    =\frac{e^{-\sigma (t-t_m)}}{\sigma}\int_{t_m}^t  \left(\sigma(s-t_m)e^{\sigma (s-t_m)}-e^{\sigma (s-t_m)}+1\right) ds
    \\
    =\frac{e^{-\tau}}{\sigma^2}\int_{0}^{\tau}  \left(\tau'e^{\tau'}-e^{\tau'}+1\right) d\tau'
    \\
    =\frac{e^{-\tau}}{\sigma^2} \left(\tau + (\tau - 2)e^{\tau} + 2\right) = (t-t_m)^2\frac{\tau e^{-\tau} + 2e^{-\tau}+ \tau - 2}{\tau^2} .
\end{gather}

Let 
\begin{equation}
    \beta_1(\tau) := \frac{ 1-e^{-\tau} - \tau e^{-\tau}}{\tau}, \quad\quad\quad \beta_2(\tau) = \frac{\tau e^{-\tau} + 2e^{-\tau}+ \tau - 2}{\tau^2}.
\end{equation}
Then the estimate can be written
\begin{equation}
    \norma{\nabla_x \partial_{\theta}\psicm{m}(t)} 
    \leq (t-t_m)\beta_1(\tau(t)) \norma{D_x^2 g} +  ((t-t_m)t_m\beta_1(\tau(t))  + (t-t_m)^2\beta_2(\tau(t)) )\norma{D_x^2 q}_{\infty}.
\end{equation}
At the endpoint of the time interval, this becomes
\begin{equation}\label{eqn:angle_at_end}
    \norma{\nabla_x \partial_{\theta}\psicm{m}^-(t_{m+1})} 
    \leq \Delta t\beta_1(\sigma \Delta t) \norma{D_x^2 g} +  (m\Delta t^2\beta_1(\sigma \Delta t)  + \Delta t^2\beta_2(t_{m+1}))\norma{D_x^2 q}_{\infty}.
\end{equation}
Integrating once more in time, we have (after some tedious calculus that I used a computer to help with)
\begin{gather}
    \int_{t_m}^t (s-t_m)\beta_1(\tau(s)) ds = (t-t_m)^2\beta_2(\tau(t)) ,
    \\
    \int_{t}^{t_m} (s-t_m)^3 \beta_2(\tau(s)) ds = (t-t_m)^3 \beta_3(\tau(t)) , 
    \\
    \beta_3(\tau(t))  = \frac{\tau^2-4\tau - 2\tau e^{-\tau} + 6 - 6e^{-\tau}}{\tau^3}.
\end{gather}
Thus,
\begin{equation}
    \int_{t_m}^{t}\norma{\nabla_x \partial_{\theta}\psicm{m}(t)} 
    \leq (t-t_m)^2\beta_2(\tau(t)) \norma{D_x^2 g} +  ((t-t_m)^2t_m\beta_2(\tau(t))  + (t-t_m)^3\beta_3(\tau(t)) )\norma{D_x^2 q}_{\infty}.
\end{equation}
\begin{equation}\label{eqn:angle_over_interval}
    \int_{t_m}^{t_{m+1}}\norma{\nabla_x \partial_{\theta}\psicm{m}(t)} 
    \leq \Delta t^2\beta_2(\sigma \Delta t) \norma{D_x^2 g} +  (\Delta t^2t_m\beta_2(\sigma \Delta t)  + \Delta t^3\beta_3(\sigma \Delta t) )\norma{D_x^2 q}_{\infty}.
\end{equation}

%_______________________________________________________________


%section ends
%_______________________________________________________________________________________________________________________________________________________

==> sections/name.tex <==
\begin{subequations}
  \begin{align}
    &\e\partial_t\Psi_{{\mathrm{u}},m}^{\e,N}+\Omega\cdot\nabla_x\Psi_{{\mathrm{u}},m}^{\e,N}+\frac{\sigma}{\e}\Psi_{{\mathrm{u}},m}^{\e,N}=\e q,
      \label{eq:hybrid_intervals_PN_uncollided}\\
    &\e\partial_t\Psi_{\mathrm{c},m}^{\e,N}+\cP_N\left(\Omega\cdot\nabla_x\Psi_{\mathrm{c},m}^{\e,N}\right)+\frac{\sigma}{\e}\Psi_{\mathrm{c},m}^{\e,N}=\frac{\sigma}{\e}(\overline{\Psi_{\mathrm{u},m}^{\e,N}}+\overline{\Psi_{\mathrm{c},m}^{\e,N}}),
     \label{eq:hybrid_intervals_PN_collided}\\\\
    &\left.\Psi_{\mathrm{c},m}^{\e,N}\right|_{t=t_m}=0, \quad \left.\Psi_{\mathrm{u},m}^{\e,N}\right|_{t=t_m}=
   \begin{cases}
   g, &\quad m = 0,\\
   \Psi_{\mathrm{u},m-1}^{\e,N}(t^-_m) + \Psi_{\mathrm{c},m-1}^{\e,N}(t^-_m) &\quad m > 0.
   \end{cases}
    \label{eq:hybrid_intervals_PN_remap_transport}
    \end{align}
        \label{eq:hybrid_intervals_PN_transport}%
    \end{subequations}

==> sections/pn.tex <==
\section{Preliminaries (notion of solutions)}
\todo{Move this earlier, when we introduce the equations}
We now recall some existence and uniqueness results for the generic problem,
\begin{align}\label{eq:general_evolution}
 &\e\partial_t\phi+\Omega\cdot\nabla_x\phi+\frac{\sigma} {\e}\phi=K\overline{\phi} + Q, \quad \text{ for } t \in (0,T),  \quad 
 \\
 &\phi(t_0) = \phi_0,\notag
 \end{align}
 with $K \in L^{\infty}(X)$, $K\geq 0$.
We adapt a result from \cite[Chapter XXI, Theorem 3]{lions1984}, which states the conditions for existence and uniqueness of mild and strong solutions to \eqref{eq:general_evolution}. We seek solutions in the space
\begin{equation}
    W_p = \left\{ \phi \in L^p((0,T);\mathbb{T}^3\times \sphe)\, |\, \partial_t \phi + \frac{1}{\e}\Omega\cdot\nabla \phi \in L^p((0,T);\mathbb{T}^3\times \sphe) , \quad \phi(0) \in L^p(\mathbb{T}^3\times \sphe)  \right\}.
\end{equation}
\begin{ass}\label{ass:regularity}
We now state the two sets of assumptions we consider.
\begin{enumerate}[A)]
    \item \label{ass:weak} $\phi_0 \in L^p(\mathbb{T}^3\times \sphe)$, and $Q\in L^p((0,T);L^p(\mathbb{T}^3\times\sphe))$ for $p \in [1,\infty)$.
    \item The assumptions in part \ref{ass:weak}, plus \label{ass:strong} $\Omega \cdot \nabla_x\phi_0 \in L^2(\mathbb{T}^2\times \sphe)$, and $Q\in C^1([0,T];L^2(\mathbb{T}^3\times\sphe))$.
\end{enumerate}
\end{ass}
\todo{verify for periodic domain.}
\begin{thm}
Given Assumption \ref{ass:regularity}.\ref{ass:weak}, there is a unique mild solution $\phi \in W_p$  with $$\phi \in C([0,T];L^p(\mathbb{T}^3\times \sphe)).$$ 
If additionally Assumption \ref{ass:regularity}.\ref{ass:strong} holds, $\phi$ is a strong solution, and
\begin{equation} 
    \phi \in C^1([0,T];L^p(\mathbb{T}^3\times \sphe)), \quad \Omega \cdot \nabla_x \phi \in C([0,T];L^p(\mathbb{T}^3\times \sphe)).
\end{equation}
\end{thm}
\subsection{Stability results}

%\subsection{$\mathrm{P}_N$ Stability} \label{sec:PN_stability}

% \begin{lem}\todo{Redundacy between this and lemma 2}
% \begin{equation}
% \label{eq:transport_stability}
%     \norma{\psi(t)}\leq \norma{g}+\int_{t_0}^t\norma{q(s)}\,ds.
% \end{equation}
% \begin{equation}
% \label{eq:pn_stability}
%     \norma{\psi^N(t)}\leq \norma{\cP^N g}+\int_{t_0}^t\norma{\cP_N q(s)}\,ds.
%     \end{equation}
% \end{lem}
% \begin{proof}
% Multiplying \eqref{eq:transp_simple} by $\psi$, integrating both in space and angle, and applying of Cauchy-Schwarz inequality gives
% \begin{equation}
%     \frac12 \p_t \norma{\psi}^2+\sigma\norma{\widetilde{\psi}}^2
%     % = \int \overline{q} \overline \psi d \Omega d \psi 
%     % = \int \widetilde q \overline \psi d \Omega d \psi 
%      = \int   \psi q d \Omega d \psi 
%     \leq \norma{q}\norma{\psi}
% \end{equation}
% Assuming $\|\psi\| \ne 0$, we can divide through by $\|\psi\|$ to obtain.
% \begin{equation}
%     \frac{d}{dt}\norma{\psi}\leq \norma{q},
% \end{equation}
% Direct integration in time gives \eqref{eq:transport_stability}.  The derivation of \eqref{eq:pn_stability} from \eqref{eq:pn} follows from the same calculation.
% \end{proof}


\todo{Rigorously justify this, include spatial derivatives}
 \begin{lem}[Stability Estimates]\label{lem:basic_stability_result} (Add sufficient assumptions for semi-group solution to exist)
\begin{enumerate}[(a)]
    \item Let  $\phi$ be the solution to
 \label{lem:unc}
 \begin{equation}
 \e\partial_t\phi+\Omega\cdot\nabla_x\phi+\frac{\sigma} {\e}\phi=Q, \quad \phi(t_0) = \phi_0.\label{eq:gen_uncollided}
 \end{equation}
Then we have
 \begin{equation}\label{eq:unc_strong}
     \|\phi(t)\| \leq e^{-\sigma(t-t_0)/\e^2}\|\phi_0\| + \cA_{t_0}(t)\|Q\|.
 \end{equation}
   \item Let  $\phi$ be the solution to
 \label{lem:coll}
 \begin{equation}
 \e\partial_t\phi+\Omega\cdot\nabla_x\phi+\frac{\sigma} {\e}\phi=\frac{\sigma} {\e}\overline{\phi} +Q, \quad \phi(t_0) = \phi_0.
 \end{equation}
Then we have
 \begin{equation}
     \|\phi(t)\| \leq \|\phi_0\| + \frac{1}{\e}\int_{t_0}^t\|Q(\tau)\|d\tau.
 \end{equation}
\end{enumerate}
  \end{lem}
 \begin{proof}
 Prove for strong case first by using greens formula for $W_2$, differentiate result in time because of $C^1$, apply gronwall. Then use density of the domain to say the same for mild solutions. Ignore the rest of this proof for now.
 
 
 To prove part (\ref{lem:unc}), we first assume Assumption \ref{ass:regularity}.\ref{ass:weak} so that the equation has a mild solution satisfying
 \begin{equation}
     \phi\left(t,x+\frac{\Omega}{\e}t, \Omega\right) = e^{-\sigma(t-t_0)/\e^2}\phi_0(x, \Omega) +\frac{1}{\e} \int_{t_0}^t e^{-\sigma(t-\tau)/\e^2}Q\left(\tau, x+\frac{\Omega}{\e}\tau,\Omega\right) d\tau.
 \end{equation}
 Taking the $L^2(\mathbb{T}^3,\sphe)$ norm   of both sides, using triangle inequality on the right hand side, and noting that $\int_{\mathbb{T}^3} f(x+v) dx =\int_{\mathbb{T}^3} f(x) dx$ by periodicity show \eqref{eq:unc_weak}.
 
 If Assumption \ref{ass:regularity}.\ref{ass:strong} holds, $\phi$ is a strong solution. We may take the inner product of the equation with $\phi$, and apply Cauchy-Schwarz and Lemma \ref{lem:diff_bd} to get \eqref{eq:unc_strong}.
 
 To prove part (\ref{lem:coll}), we note from the proof of part (\ref{lem:unc}) that a mild solution must satisfy
  \begin{gather}
     \phi\left(t,x+\frac{\Omega}{\e}t, \Omega\right) = e^{-\sigma(t-t_0)/\e^2}\phi_0(x, \Omega) + \int_{t_0}^t e^{-\sigma(t-\tau)/\e^2}Q\left(\tau, x+\frac{\Omega}{\e}\tau,\Omega\right) d\tau
    \\ + \int_{t_0}^t e^{-\sigma(t-\tau)/\e^2}\overline{\phi}\left(\tau, x+\frac{\Omega}{\e}\tau,\Omega\right) d\tau.
 \end{gather}
 We again take the $L^2(\mathbb{T}^3,\sphe)$ norm of both sides, apply the triangle inequality, and noting that
 \begin{gather}
      \int_{\sphe}\int_{\mathbb{T}^3}\left(\int_{t_0}^t e^{-\sigma(t-\tau)/\e^2}\overline{\phi}\left(\tau, x+\frac{\Omega}{\e}\tau,\Omega\right) d\tau \right)^2 dx d\Omega =  \int_{\sphe}\int_{\mathbb{T}^3}\left(\int_{t_0}^t e^{-\sigma(t-\tau)/\e^2}\overline{\phi}\left(\tau, x,\Omega\right) d\tau \right)^2 dx d\Omega
      \\
      \int_{t_0}^t e^{-2\sigma(t-\tau)/\e^2}d\tau \int_{\sphe}\int_{\mathbb{T}^3}\int_{t_0}^t \overline{\phi}\left(\tau, x,\Omega\right)^2 d\tau  dx d\Omega = \left( 1 - e^{-2\sigma(t-t_0)/\e^2} \right)\int_{\sphe}\int_{\mathbb{T}^3}\int_{t_0}^t \overline{\phi}\left(\tau, x,\Omega\right)^2 d\tau  dx d\Omega
      \\
      \left( 1 - e^{-2\sigma(t-t_0)/\e^2} \right)\int_{\sphe}\int_{\mathbb{T}^3}\int_{t_0}^t \phi\left(\tau, x,\Omega\right)^2 d\tau  dx d\Omega
 \end{gather}
 Not sure that's going anywhere...maybe have to do youngs?...$L^1$ could work...but the strong case works out.
 \end{proof}
 The same results exist for $P_N$ discretizations with the data replaced by $\cP_N$. The proofs are almost exactly the same.
%  \begin{lem}[Basic Stability Results]\label{lem:basic_stability_result_old} Let $\varphi,\,\zeta \in C^{1}([t_0,T];C^1(\mathbb{T}^3)\cap L^2(\sphe))$  satisfy the following PDEs  
%  \begin{equation}
%  \partial_t\zeta+\Omega\cdot\nabla_x\zeta+\sigma \zeta=Q,
%  \end{equation}
%  \begin{equation}
%  \partial_t\varphi+\Omega\cdot\nabla_x\varphi+\sigma \varphi=\sigma\overline{\varphi}+Q,
%  \end{equation} 
%  respectively, with $Q\in C([t_0,T];L^2(\mathbb{T}^3\times\sphe))$, and consider $\phi\in C^{1}([t_0,T];C^1(\mathbb{T}^3)\cap\Pi^N(\sphe))$
%  \begin{equation}
%      \partial_t\phi+P_N(\Omega\cdot\nabla_x\phi)+\sigma \phi=\sigma\overline{\phi}+Q_N
%  \end{equation}
%  and $Q_N\in C([t_0,T];L^2(\mathbb{T}^3)\cap \Pi^N(\sphe))$. We will assume periodic boundary conditions in the space variable in all the above equations, then for all $t\in [t_0,T]$,
%  \begin{enumerate}[I.]
%      \item \begin{equation*}
%      \norma{\zeta(t)}\leq e^{-\sigma(t-t_0)}\norma{\zeta(t_0)}+\int_{t_0}^te^{-\sigma(t-s)}\norma{Q(s)}\,ds.
%      \end{equation*} 
%      \item \begin{equation*}
%      \norma{\varphi(t)}\leq \norma{\varphi(t_0)}+\int_{t_0}^t\norma{Q(s)}\,ds.
%      \end{equation*}
%      \item\label{lem:dis}\begin{equation*}
%      \norma{\phi(t)}\leq \norma{\phi(t_0)}+\int_{t_0}^t\norma{Q_N(s)}\,ds.
%      \end{equation*}
%  \end{enumerate}
%  \end{lem}
%  \begin{proof}
%  \textbf{Proof of \ref{lem:unc}}: If we multiply by $\zeta$ in \eqref{eq:gen_uncollided}, integration in both space and angle and an application of Cauchy-Schwarz inequality gives us
%  \begin{equation*}
%      \frac{d}{dt}\norma{\zeta}+\sigma\norma{\zeta}\leq\norma{Q},
%  \end{equation*}
%  the conclusion follows by Gronwall's inequality.

% \textbf{Proof of \ref{lem:coll}}: 
% Notice that $\varphi$ also satisfies
% \begin{equation*}
%      \partial_t\varphi+\Omega\cdot\nabla_x\varphi+\sigma \widetilde{\varphi}=Q,
% \end{equation*}
%  now multiplying by $\varphi$ and integrating both in space and velocity space and an application of Cauchy-Schwarz inequality, gives us
%  \begin{equation*}
%      \frac{1}{2}\frac{d}{dt}\norma{\varphi}^2+\sigma\norma{\widetilde{\varphi}}^2\leq \norma{Q}\norma{\varphi}
%  \end{equation*}
%  then 
%  \begin{equation*}
%      \frac{d}{dt}\norma{\varphi}\leq \norma{Q},
%  \end{equation*}
%  direct integration allow us to conclude.

%  \textbf{Proof of \ref{lem:dis}}: The proof is the same line by line as in \ref{lem:coll}, since the definition of $P_N$ implies
%  \begin{equation*}
%      \langle P_N(\Omega\cdot\nabla_x\phi),\phi\rangle=\langle(\Omega\cdot\nabla_x\phi),\phi\rangle=0.
%  \end{equation*}
%  \end{proof}
% % %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Now with this Lemma we are able to show the following stability results for both $\psi$ and $\psi^N$,
%  \todo{Check if we use this anywhere}
%  \begin{lem}[Non-splitting Bound]\label{lem:nonsplitting_bound} 
%  Let $\alpha_x$ be a multi-index for the partial derivatives with respect to $x$, $\psi$ be the solution to \eqref{eq:scaled_transp}, and let us assume that this solutions are smooth with respect to $x$, then 
%  \begin{equation}
%      \norma{\psi_{\alphax}(t)}\leq \norma{g_{\alphax}}+t\norma{q_{\alphax}}_{\infty}.\label{eq:nonsplitting_bound}
%  \end{equation}
%  \end{lem}
%  \begin{proof}
%  Notice that by taking partial derivative $\partial_{\alphax}$ in \eqref{eq:scaled_transp} we obtain, 
%  \begin{equation*}
%      \partial_t\psi_{\alphax}+\Omega\cdot\nabla_x\psi_{\alphax}+\sigma\psi_{\alphax}=\sigma\overline{\psi_{\alphax}}+q_{\alpha_x},
%  \end{equation*}
%  then we apply Lemma \ref{lem:basic_stability_result}, part \ref{lem:coll}, with $t_0=0$, $\varphi=\psi_{\alpha_x}$ and $Q=q_{\alpha_x}$.
%  \end{proof}
%  \begin{thm}[Long time $L^2$ stability of the non-splitting discretization\label{thm:stability_nonsplitting_discrete}] For $t\in[0,T)$, we have
%  \begin{equation}
%  \norma{\psi^N(t)} \leq\norma{P_Ng} + t\norma{P_Nq}_{\infty},
%  \end{equation}
%  \end{thm}
%  \begin{proof}
%  This is just another application of  Lemma \ref{lem:basic_stability_result}, we use part \ref{lem:dis} with $t_0=0$, $\phi=\psi^N$ and $Q_N=P_Nq$, we conclude.
%  \end{proof}


==> sections/stabilty.tex <==






==> sections/timestep.tex <==
\section{How to pick $\Delta t$}
In this section, we obtain error estimates for the $P_N$ discretizations of the transport and hybrid model that are in terms of problem data. These estimates yield insight into how often the the remap should be performed (the size of $\Delta t$) to obtain comparable accuracy with the non-split discretization.
The error analysis performed in Sections \ref{sec:pn_error}-\ref{sec:hybrid_error} can now be combined with the interpolation error estimates in Sections \ref{sec:angle_reg_transport}-\ref{sec:angle_reg_hybrid}.
\begin{thm}
Let $\psi$ be the solution to \eqref{eq:scaled_transp}, and assume $\psi\in C^1([0,T]; C^{3}(X)\cap H^1(\mathbb{S}^2))$. Then
	\begin{equation}
		\norma{e^N(t)}\leq \frac{CE_\sigma(t)}{N},
		\label{eq:non_splitting_error}
	\end{equation}
here $C$ is independent of $\sigma$ and $N$, and 
\begin{equation}
    E_\sigma(t)=E_{\sigma,1}(t)+E_{\sigma,2}(t)
\end{equation}
\begin{equation}
    E_{\sigma,1}(t)\coloneqq \max_{i,j}\norma{\partial_{\theta_{i,j}}g}\kappa(t)+\left[\norma{\partial_x g}+\max_{i,j}\norma{\partial_{\theta_{i,j}}q}_{\infty}\right]\gamma(t)t+\norma{\partial_x q}_{\infty}\left[1-\gamma(t)\right]\frac{t}{\sigma}
\end{equation}
and 
\begin{equation}
    E_{\sigma,2}(t)\coloneqq\max_{i,j}\norma{\nabla_x\partial_{\theta_{i,j}}g}\gamma(t)t+\left[\norma{D^2_xg}+\max_{i,j}\norma{\nabla_x\partial_{\theta_{i,j}}q}_{\infty}\right]\Gamma(t)+\norma{D^2_x q}_{\infty}\left[t^2-\Gamma(t)\right]/\sigma,
\end{equation}
where
\begin{equation}
    \Gamma(t)\coloneqq \int_0^t \gamma(\omega)\omega\,d\omega.
\end{equation}
\end{thm}
\begin{proof}
First of all, by Lemma \ref{lem:approx_prop},  and an application of Lemma \ref{lem:nonsplitting_reg},
\begin{align*}    
\norma{\eta^N}^2&=\int_{\mathbb{T}^3}\norma{\eta^N}_{L^2(\sphe)}^2\,dx\\
&\lesssim N^{-2}\int_{\mathbb{T}^3}|\psi|_{H^1(\sphe)}^2\,dx\\
&\lesssim N^{-2}\sum_{1\leq i,j\leq 3}\int_{\mathbb{T}^3}\norma{\partial_{\theta_{i,j}}\psi}_{L^2(\sphe)}^2\,dx\\
&\lesssim N^{-2}\sum_{1\leq i,j\leq 3}\norma{\partial_{\theta_{i,j}}\psi}^2\\
&\lesssim N^{-2}\left(E_{\sigma,1}(t)\right)^2
\end{align*}
Analogously, another application of Lemma \eqref{lem:nonsplitting_reg}
\begin{align*}    
\norma{\nabla_x\eta^N}^2&\lesssim N^{-2}\sum_{1\leq i,j\leq 3}\norma{\nabla_x\partial_{\theta_{i,j}}\psi}^2\\
&\lesssim N^{-2}[\max_{i,j}\norma{\nabla_x\partial_{\theta_{i,j}} g}\kappa(t)+\left[\norma{D^2_xg}+\max_{i,j}\norma{\nabla_x\partial_{\theta_{i,j}}q}_{\infty}\right]\gamma(t)t+\norma{D^2_xq}_{\infty}\left[1-\gamma(t)\right]\frac{t}{\sigma}]^2,
\end{align*}
then by Lemma \ref{lem:galerkin_non_splitting_estimate}, we trivially have
\begin{equation*}
    \norma{e^N(t)}\leq \norma{\eta^N}+\norma{\xi^N}\leq \norma{\eta^N}+\int_{0}^t\norma{\nabla_x\eta^N(\omega)}\,d\omega.
\end{equation*}
The conclusion follows by putting together all the above calculations and integration.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Hybrid}


If the hybrid solution is smooth enough, we can combine the error and regularity estimates to obtain
\begin{gather}
\norma{e^N(T)}\leq \frac{C}{N} \sum_{j=0}^{m}\left[\norma{\partial_{\theta}\psicm{m}^{N,-}(t_{j+1})}+\int_{t_j}^{t_{j+1}}\norma{\partial_{\theta}\nabla_x\psicm{m}^{N,-}(s)}\,ds\right]
\\
\leq \frac{C}{N} \sum_{j=0}^{m} \left( \Delta t\beta_1(\sigma \Delta t) \norma{\nabla_x g} +  (j\Delta t^2\beta_1(\sigma \Delta t)  + \Delta t^2\beta_2(\sigma \Delta t) )\norma{\nabla_x q}_{\infty}\right)
\\
 +  \frac{C}{N} \sum_{j=0}^{m} \left( \Delta t^2\beta_2^{(m)}\norma{D_x^2 g} +  (j\Delta t^3\beta_2^{(m)} + \Delta t^3\beta_3(\sigma \Delta t) )\norma{D_x^2 q}_{\infty}\right)
 \\
\sim \frac{C}{N}\left( T\beta_1(\sigma \Delta t) \norma{\nabla_x g} +  (\frac{T^2}{2}\beta_1(\sigma \Delta t)  + \Delta t T\beta_2(\sigma \Delta t) )\norma{\nabla_x q}_{\infty}\right)
\\
 +  \frac{C}{N}  \left( \Delta t T \beta_2(\sigma \Delta t) \norma{D_x^2 g} +  (\frac{\Delta t T^2}{2}\beta_2(\sigma \Delta t)  + \Delta t^2T\beta_3(\sigma \Delta t) )\norma{D_x^2 q}_{\infty}\right).
\end{gather}





\subsection{Putting the results next to eachother}
Assume that the initial conditions and q are isotropic. Smooth enough. At the final time, the error for the $P_N$ equations is
\begin{gather}
    \norma{e^N(T)}\leq \frac{C}{N}\left( T\gamma(T) \norma{\nabla_x g}+\left[1-\gamma(T)\right]\frac{T}{\sigma}\norma{\nabla_x q}_{\infty}\right)
    \\
    +\frac{C}{N}\left(\Gamma(T) \norma{D^2_xg}+\left[T^2-\Gamma(T)\right]/\sigma\norma{D^2_x q}_{\infty} \right)
\end{gather}

The hybrid result is.
\begin{gather}
\norma{e^N(T)}\leq \frac{C}{N}\left( T\beta_1(\sigma \Delta t) \norma{\nabla_x g} +  (\frac{T^2}{2}\beta_1(\sigma \Delta t)  + \Delta t T\beta_2(\sigma \Delta t) )\norma{\nabla_x q}_{\infty}\right)
\\
 +  \frac{C}{N}  \left( \Delta t T \beta_2(\sigma \Delta t) \norma{D_x^2 g} +  (\frac{\Delta t T^2}{2}\beta_2(\sigma \Delta t)  + \Delta t^2T\beta_3(\sigma \Delta t) )\norma{D_x^2 q}_{\infty}\right).
\end{gather}
Note that when $\sigma \Delta t$ is large, $\beta_1 \sim \beta_2 \sim \beta_3 \sim (\sigma \Delta t)^{-1}$. When $\sigma T$ is large, $\gamma \sim (\sigma T)^{-1}$. When that product is small,
\begin{equation}
    \beta_n(\sigma \Delta t) = \frac{\sigma \Delta t}{(n+1)!} + \mathcal{O}((\sigma \Delta t)^2).
\end{equation}
\begin{equation}
    \gamma(\sigma T) = \sigma T + \mathcal{O}((\sigma T)^2)
\end{equation}
\end{proof}
%_______________________________________________________________________________________________________________________________________________________
